Symbolic Regression on Sparse and Noisy Data with Gaussian Processes

In this paper, we address the challenge of deriving dynamical models from sparse and noisy data. High-quality data is crucial for symbolic regression algorithms; limited and noisy data can present modeling challenges. To overcome this, we combine Gaussian process regression with a sparse identification of nonlinear dynamics (SINDy) method to denoise the data and identify nonlinear dynamical equations. Our approach GPSINDy offers improved robustness with sparse, noisy data compared to SINDy alone. We demonstrate its effectiveness on simulation data from Lotka-Volterra and unicycle models and hardware data from an NVIDIA JetRacer system. We show superior performance over baselines including more than 50% improvement over SINDy and other baselines in predicting future trajectories from noise-corrupted and sparse 5 Hz data.

==> sections/methods_dx_A.tex <==

\textbf{Smoothing $\dot{\boldsymbol{X}}$:} Similarly, the joint distribution of the training and test points for the state derivatives $ \dot{ \boldsymbol{X} } $ is given by 
% 
\begin{equation}
\begin{bmatrix}
\dot{\boldsymbol{X}}_{*} \\
\dot{\boldsymbol{X}}
\end{bmatrix} 
\! \sim  
\mathcal{N} 
\Bigg( 
\! 
\begin{bmatrix}
0 \\ 
0 
\end{bmatrix}\! , \! 
\begingroup % keep the change local
\setlength\arraycolsep{1pt}
% \begin{bmatrix}
% K(\boldsymbol{X}_{*}, \boldsymbol{X}_{*}) \! & K(\boldsymbol{X}_{*}, \boldsymbol{X}) \\
% K(\boldsymbol{X}, \boldsymbol{X}_{*})  \! &  K(\boldsymbol{X},\boldsymbol{X}) + \sigma_n^2 I 
% \end{bmatrix}
\begin{bmatrix}
K(\boldsymbol{X}_{*}, \boldsymbol{X}_{*}) \! & K(\boldsymbol{X}_{*}, \boldsymbol{X}) \\
K(\boldsymbol{X}, \boldsymbol{X}_{*})  \! &  K(\boldsymbol{X},\boldsymbol{X}) + \sigma_n^2 I 
\end{bmatrix}
\! 
\bigg) ,
\endgroup
\end{equation}
% 
where $K(\boldsymbol{X},\boldsymbol{X}_*)$ denotes the $ r \times r_* $ matrix of the covariances and similarly for $K(\boldsymbol{X},\boldsymbol{X})$, $ K(\boldsymbol{X}_*, \boldsymbol{X}) $ and $K(\boldsymbol{X}_*, \boldsymbol{X}_*)$. 
% 
$ \sigma_n $ is the noise variance hyperparameter for $ \dot{\boldsymbol{X}} $. 
% 
% The kernel for $ \dot{\boldsymbol{{X}}} $ is characterized by its tunable hyperparameters: $ \sigma_f $ (signal variance) and $ \sigma_l $ (length scale) 
The choice of kernel for $ \dot{\boldsymbol{{X}}} $ can also be determined by evaluating its marginal log-likelihood 
% 
\begin{equation}
    \begin{aligned}
    -\operatorname{log} p(\dot{\boldsymbol{X}})  = & \, 
    \frac{1}{2}  
    \big( \dot{\boldsymbol{X}} - m(\boldsymbol{X}) \big) ^{\top} (K + \sigma_n^2 )^{-1} \big( \dot{\boldsymbol{X}} 
    \\ 
    & 
    - m(\boldsymbol{X}) \big) 
    + \frac{1}{2} \operatorname{log} | K | 
    + \frac{n}{2} \operatorname{log} (2 \pi).  
    \end{aligned}
    \label{eq:Xdot_marg_likelihood}
\end{equation} 
% 
% \begin{equation}
%     k(  \boldsymbol{X}_i, \boldsymbol{X}_j ) = \sigma_f^2 \exp \big( - \frac{1}{2 \sigma_l^2} || \boldsymbol{X}_i - \boldsymbol{X}_j || ^2 \big).
% \end{equation}
% 
and choosing the kernel that minimizes the negative log-likelihood score. To calculate smoothed estimates of $\dot{\boldsymbol{X}}$ evaluated at the test points $\boldsymbol{X}_*$, we compute the posterior mean 
% 
\begin{equation}
    \dot{\boldsymbol{X}}_{GP} = K(\boldsymbol{X}_{*}, \boldsymbol{X}) [ K(\boldsymbol{X},\boldsymbol{X}) + \sigma_n^2 I ]^{-1} \, \dot{\boldsymbol{X}} .
    \label{eq:Xdot_GP}
\end{equation}
% 
We note that $ \dot{\boldsymbol{X}}_{GP} $ can also be computed using the smoothed or interpolated measurements $ \boldsymbol{X}_{GP} $ via 
\begin{equation}
    \dot{\boldsymbol{X}}_{GP} = K(\boldsymbol{X}_{GP*}, \boldsymbol{X}_{GP}) [ K(\boldsymbol{X}_{GP},\boldsymbol{X}_{GP}) + \sigma_n^2 I ]^{-1} \, \dot{\boldsymbol{X}} .
    \label{eq:Xdot_GP_X_GP}
\end{equation}
% 
Now that we have shown how to obtain  
% the smoothed estimates of the state 
$ \boldsymbol{X}_{GP} $ and $ \dot{\boldsymbol{X}}_{GP} $, we move forward to solve the problem in \eqref{eq:sindy}. 
% 
% 
\begin{remark}
% 
The novelty of our method lies in how 
we treat $ \boldsymbol{X}_{GP} $ or $ \boldsymbol{U} $ as the input to the kernel for estimating $ \dot{\boldsymbol{X}} $. 
% 
This approach can produce smoothed and interpolated state derivatives $ \dot{\boldsymbol{X}}_{GP} $ for symbolic regression. 
% 
\end{remark}

\subsection{GPSINDy: Symbolic Regression with GP Denoising} 
% 
% First, we minimize the negative log-likelihood of the state $ \boldsymbol{X} $ with respect to the hyperparameters $ \boldsymbol{\theta} = [ \theta_f, \theta_l, \theta_n ] $, assuming its mean function $m(t) = 0$ via Equation \eqref{eq:gp_marg_likelihood}. 
\textbf{Kernel cross-validation:} 
% To compute the smoothed state estimates $\boldsymbol{X}_{GP}$, 
We evaluate the marginal log-likelihood of the state $\boldsymbol{X}$ using the SE, Mat\'ern 1/2, Mat\'ern 3/2, periodic, and RQ kernels via Equation \eqref{eq:gp_marg_likelihood} and optimize the hyperparameters for each respective kernel. 
% 
We select the kernel with the highest positive marginal log-likelihood score to compute $\boldsymbol{X}_{GP}$ via Equation \eqref{eq:X_GP}.  

minimize the negative log-likelihood of the state $ \boldsymbol{X} $ with respect to the hyperparameters $ \boldsymbol{\theta} = [ \theta_f, \theta_l, \theta_n ] $, assuming its mean function $m(t) = 0$ via Equation \eqref{eq:gp_marg_likelihood}. 
% 
We 
% 
% Then, we condition the distribution of the training data on the test data to obtain the posterior mean of the state evaluated at the test points $\boldsymbol{t}_*$ according to \eqref{eq:X_GP}. 
Then, we compute $\boldsymbol{X}_{GP}$ via \eqref{eq:X_GP}. 
% 

Next, we minimize the negative log-likelihood of the state derivative $ \dot{\boldsymbol{X}} $ with respect to the hyperparameters $\sigma_f$, $\sigma_l$, and $\sigma_n$ as in  \eqref{eq:Xdot_marg_likelihood}. 
% \red{ that is our method: we are doing a fancy prediction of state derivatives, by using the state X in our kernel of the state-derivatives. in the cost function of the log likelihood of our derivatives. that allows us to predict dynamical systems nicely. } 
% The negative log-likelihood of the data $\dot{\boldsymbol{X}}$ 
% which is given by 
% 
where $ K = k( \boldsymbol{X}_{GP}, \boldsymbol{X}_{GP} ) 
 $. Again, we assume a mean function $ m( \boldsymbol{X} ) = 0 $. 
% 
Then, we compute the posterior mean $ \dot{\boldsymbol{X}}_{GP} $ using Equation \eqref{eq:Xdot_GP_X_GP}. 
% 

\textbf{LASSO:} Finally, we update the LASSO problem from \eqref{eq:sindy} to use 
% the smoothed states 
$ \boldsymbol{X}_{GP} $ 
and 
% derivatives 
$ \dot{\boldsymbol{X}}_{GP} $ when solving for the coefficients of the system dynamics 
% 
\begin{equation}
    \bxi_j = \argmin_{\boldsymbol{\xi} \in \mathbb{R}^{p}} \norm*{ \boldsymbol{\Theta}(\boldsymbol{X}_{GP}, \boldsymbol{U})^{\top} \boldsymbol{\xi} - \dot{\boldsymbol{X}}_{GP, j}  }_2 + \lambda \norm*{ \bxi }_1 ,  
    \label{eq:gpsindy} 
\end{equation} 
% 
where $ \dot{\boldsymbol{X}}_{GP, j} $ represents the $j^{\rm th}$ column of $ \dot{\boldsymbol{X}}_{GP} $. 
% 
% \begin{remark}
% We can evaluate $ \boldsymbol{X}_{GP} $ at the test points of the input data or interpolate along a $ \boldsymbol{t}_* $ of higher frequency. Kriging gives the best linear unbiased estimates at unsampled locations for spatial and
% temporal variables\cite{rasmussen_gps}, which can be leveraged to increase the data inputs for symbolic regression. Likewise, $ \dot{ \boldsymbol{X} }_{GP} $ can be interpolated from $ \boldsymbol{X}_{GP} $. 
% \end{remark}

==> sections/old/old_methods.tex <==

\violet{
Our key innovation is to embed the sparse regression problem from SINDy within a non-parametric Gaussian process framework. 
More specifically, we identify the mean function from Gaussian processes $m(\mathbf{x})$ with the expression from SINDy $ \bThx \bXi $. The measurements $\state$ correspond with the state derivative matrix $\bdX$. 
}

% In this work, we combine symbolic regression \david{just choose a term. is it symbolic regression, LASSO, or SINDy?} with the noise reduction capability of Gaussian processes. Just like in SINDy, 
% we first obtain a time-history \david{see earlier comment} of the state and its derivatives \david{why plural?}. 
% We arrange the data into two matrices \david{these constructions belong wherever the variables are introduced, whether that is here or in preliminaries}

% \begin{equation}
%     \mathbf{X} = 
%     \begin{bmatrix}
%         x_1(t_1) & x_2(t_1) & \ldots    & x_n(t_1) \\ 
%         x_1(t_2) & x_2(t_2) & \ldots    & x_n(t_2) \\ 
%         \vdots   & \vdots   & \ddots    & \vdots   \\ 
%         x_1(t_m) & x_2(t_m) & \ldots    & x_n(t_m) 
%     \end{bmatrix}
% \end{equation}

% \begin{equation}
%     \dot{\mathbf{X}} = 
%     \begin{bmatrix}
%         \dot{x}_1(t_1) & \dot{x}_2(t_1) & \ldots    & \dot{x}_n(t_1) \\ 
%         \dot{x}_1(t_2) & \dot{x}_2(t_2) & \ldots    & \dot{x}_n(t_2) \\ 
%         \vdots         & \vdots         & \ddots    & \vdots   \\ 
%         \dot{x}_1(t_m) & \dot{x}_2(t_m) & \ldots    & \dot{x}_n(t_m)
%     \end{bmatrix} 
% \end{equation}

% and then construct a library consisting of candidate nonlinear functions of the columns of $\mathbf{X}$ 

% \david{nit: use $\sin$ not $sin$}
% \begin{equation}
%     \mathbf{\Theta(x)} = 
%     \begin{bmatrix}
%         \;\vertbar & \vertbar    & \vertbar         & \vertbar         &        & \vertbar \; \\
%         \;1        & \mathbf{X}  & \mathbf{X}^{P_2} & \mathbf{X}^{P_3} & \ldots & sin(\mathbf{X}) & \ldots \; \\ 
%         \;\vertbar & \vertbar    & \vertbar         & \vertbar         &        & \vertbar \;
%     \end{bmatrix} 
% \end{equation}

% where $\mathbf{X}^{P_2}$ and $\mathbf{X}^{P_3}$ denote higher order polynomials. For instance, $\mathbf{X}^{P_2}$ is 

% \begin{equation}
%     \mathbf{X}^{P_2} = 
%     % \begingroup
%     % \setlength\arraycolsep{1pt}
%     \begin{bmatrix}
%         x_1^2(t_1) & x_1(t_1) x_2(t_1) & \ldots & x_2^2(t_1) & \ldots    & x_n^2(t_1) \\ 
%         x_1^2(t_2) & x_1(t_2) x_2(t_2) & \ldots & x_2^2(t_2) & \ldots    & x_n^2(t_2) \\ 
%         \vdots     & \vdots            &        & \vdots     & \ddots    & \vdots     \\ 
%         x_1^2(t_m) & x_1(t_m) x_2(t_m) & \ldots & x_2^2(t_m) & \ldots    & x_n^2(t_m)   
%     \end{bmatrix} . 
%     % \endgroup
% \end{equation}

% We can now set up the sparse regression problem from Eq. \ref{eq:deriv_meas}, incorporating the noise magnitude, $\mu$, and the matrix of independent and identically distributed Gaussian variables with zero mean, $\mathbf{Z}$ 
% \david{if you are repeating an equation it is a very good sign that something is organized improperly. same with (11)}

% \begin{equation}
%     \mathbf{\dot{X}} = \mathbf{\Theta(x)\Xi} + \mu \mathbf{Z} \, .  
% \end{equation}

% We would like to regress the library of candidate nonlinear terms onto the derivatives obtained from the measurements \david{nonstandard phrasing}. The problem can be expressed as thus  

% \begin{equation}
%     \mathbf{\xi}_k = \argmin_{\mathbf{\xi}} || \mathbf{\Theta(x)} \mathbf{\xi} - \mathbf{\dot{X}}_k  ||_2 + \lambda || \mathbf{\xi} ||_1 \, , 
%     \label{eq:SINDy}
% \end{equation}

% but the presence of noise results in the incorrect identification of nonlinear terms. In order to introduce our method for mitigating noise, we first define the marginal log-likelihood for Gaussian processes  
% % Before we introduce our method, we define the marginal log-likelihood for Gaussian processes 

% \begin{equation}
%     \begin{aligned}
%     \operatorname{log} p(\mathbf{y|x}) & = 
%     -\frac{1}{2}  
%     \big( \mathbf{y} - \mathbb{E}[\mathbf{y}] \big) ^T K_y^{-1} \big( \mathbf{y} - \mathbb{E}[\mathbf{y}] \big)
%     - \frac{1}{2} \operatorname{log} | K_y | 
%     - \frac{n}{2} \operatorname{log} (2 \pi) 
%     \\ 
%     K_y & = k(\mathbf{x,x}) + \sigma_n^2 I 
%     \end{aligned}
%     \label{eq:gp_marg_likelihood}
% \end{equation} 

% in which $\mathbf{y}$ is the vector of observations \david{see earlier comment about measurements and naming} and $\mathbb{E}[\mathbf{y}]$ represents its mean function \david{are you going to use $m(.)$?}. The term $( \mathbf{y} - \mathbb{E}[\mathbf{y}] )$ in Equation \ref{eq:gp_marg_likelihood} \david{not worth your time now, but the cleveref pkg i suggested in the lab writing guide is your friend} is replaced with $\mathbf{\Theta(x)} \mathbf{\xi} - \mathbf{\dot{X}}_k$ \david{the elegant way to say this is that ``A key insight of our work is that we embed the structure of the SINDy model (10) as the mean function $m(.)$ in the GP likelihood (12).'' You could also probably avoid effectively duplicating this eqn} from Equation \ref{eq:SINDy} to formulate 

% \begin{equation}
%     \begin{aligned}
%     \operatorname{log} p(\mathbf{y|x}) & = 
%     -\frac{1}{2}  
%     \big( \mathbf{\Theta(x)} \mathbf{\xi} - \mathbf{\dot{X}}_k \big) ^T K_y^{-1} \big( \mathbf{\Theta(x)} \mathbf{\xi} - \mathbf{\dot{X}}_k \big)
%     - \frac{1}{2} \operatorname{log} | K_y | 
%     - \frac{n}{2} \operatorname{log} (2 \pi) 
%     \\ 
%     K_y & = k(\mathbf{\dot{X}, \dot{X}}) + \sigma_n^2 I .  
%     \end{aligned} 
%     \label{eq:gaussian_sindy}
% \end{equation} 

\violet{
To solve for the coefficient vector for active dynamical terms, $\bxi$, 
we minimize the negative log likelihood function. The constant term $\frac{n}{2} \operatorname{log} (2\pi)$ from the GP marginal likelihood is dropped as it bears no effect on the solution, but $K$ remains the same. To promote sparsity in the solution, we add the term $\lambda || \bxi ||_1$ from SINDy, resulting in 
}
% 
\begin{equation}
    \bxi_k 
    = 
    \argmin_{\mathbf{\xi}} 
    \; 
    \frac{1}{2}  
    \big( \mathbf{\Theta(x)} \mathbf{\xi} - \mathbf{\dot{X}}_k \big) ^T K^{-1} \big( \mathbf{\Theta(x)} \bxi + \mathbf{\dot{X}}_k \big)
    + \frac{1}{2} \operatorname{log} | K |     
    + 
    \lambda 
    || \bxi ||_1 
    \, . 
    \label{eq:argmin_gaussian_sindy}
\end{equation}
% 
\violet{
Depending on the size of the dataset and the number of measured states, Equation \ref{eq:argmin_gaussian_sindy} can be computationally expensive to minimize. 
% \david{one does not ``solve'' an objective function....}. 
Fortunately, it is also separable, which makes it suitable for computational acceleration via a splitting method \citep{boyd_admm}. 
% \david{avoid calling it distributed, since we are doing everything single threaded. i'd just say ``suitable for computational acceleration via a splitting method''} 
}


% % ------------------- % 
% \subsection{Alternating Direction Method of Multipliers (ADMM)}

% \input{sections/admm}

% \subsubsection{GaussianSINDy with ADMM}

% Returning to our problem of discovering nonlinear dynamics, b
By casting $ f(x) $ as 
% 
\begin{equation}
    f(\bxi, \theta) = 
    \frac{1}{2}  
    \big( \mathbf{\Theta(x)} \mathbf{\xi} - \mathbf{\dot{X}}_k \big) ^T K_y^{-1} \big( \mathbf{\Theta(x)} \mathbf{\xi} + \mathbf{\dot{X}}_k \big)
    + \frac{1}{2} \operatorname{log} | K_y |     
\end{equation}
% 
and setting $ g(z) $ as 
% 
\begin{equation}
    g( \mathbf{z} ) = \lambda || \mathbf{z} ||_1 \; , 
\end{equation}
% 
we can reformulate Equations \ref{eq:argmin_gaussian_sindy} and \ref{eq:admm} as 
% 
\begin{equation}
    \begin{aligned}
        \operatorname{minimize}      & \; \; \; f( \mathbf{\xi}, \theta ) + g( \mathbf{z} ) \\ 
        \operatorname{subject \; to} & \; \; \; \mathbf{\xi} - \mathbf{z} = 0 . 
    \end{aligned}
\end{equation}

The augmented Lagrangian for ADMM becomes 

\begin{equation}
    L_{\rho}(\xi, \theta, \mathbf{z}, y) = f(\xi, \theta) + g(\mathbf{z}) + y^T ( \mathbf{\xi} - \mathbf{z} ) + \frac{\rho}{2}|| \mathbf{\xi} - \mathbf{z} ||_2^2  
\end{equation}


\red{Still working on ADMM pseudocode below. Algorithm \ref{alg:GaussianSINDy_ADMM}}
\david{why is it PPO....?}

\begin{algorithm}
	\caption{GaussianSINDy}
        \label{alg:GaussianSINDy_ADMM}
	\begin{algorithmic}[1]
            \State initialize k = 1 
            \For { $iteration=1,2,\ldots$ }
                \State $ \mathbf{\xi}^{k+1} := \argmin_{\xi} L_{\rho}( \xi, \theta^k, \mathbf{z}^k, y^k) $
                \State $ \mathbf{\theta}^{k+1} := \argmin_{\theta} L_{\rho}( \xi^{k+1}, \theta, \mathbf{z}^k, y^k) $
                \State $ \mathbf{z}^{k+1} := \argmin_{\mathbf{z}} L_{\rho}( \xi^{k+1}, \theta^{k+1}, \mathbf{z}, y^k) $
                \State $ y^{k+1} := y^k + \rho ( \mathbf{\xi - z} ) $
            \EndFor 
	\end{algorithmic} 
\end{algorithm}


\subsubsection{Derivatives}

Key to regressing onto the dynamics is having access to derivative data. Various ways of obtaining the derivatives including finite differencing, total variational derivatives, and treating the data set as a Gaussian process and then performing differentiation, resulting in another Gaussian process.
\david{we discussed this in person already}

\red{
In this work, the noisy data set is smoothed using Gaussian process regression, and then the derivatives are obtained by finite differencing. 
}


==> sections/results_A.tex <==


\begin{table}[!t]
\centering
\begin{tabular}{lllllll}
    \toprule
     & \multicolumn{2}{c}{Ground Truth} & \multicolumn{2}{c}{SINDy} & \multicolumn{2}{c}{GPSINDy (Ours)} \\
    \cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7}
    $\Theta$ term & $\dot{x}_{1}$ & $\dot{x}_{2}$ & $\dot{x}_{1}$ & $\dot{x}_{2}$ & $\dot{x}_{1}$ & $\dot{x}_{2}$ \\
    \midrule
    $x_{1}$                 & 1.1  & 0.0  & 1.108           & \textbf{0.0}      & \textbf{1.097}    & \textbf{0.0} \\
    $x_{2}$                 & 0.0  & -0.1 & \textbf{0.0}    & \textbf{-0.997}   & \textbf{0.0}      & -0.980 \\
    $x_{1}x_{2}$            & -0.4 & 0.4  & \textbf{-0.397} & 0.382             & -0.358            & \textbf{0.396} \\
    $x_{2}x_{2}$            & 0.0  & 0.0  & \textbf{0.0}    & \textbf{0.0}      & \textbf{0.0}      & -0.005 \\
    $\cos(x_{1})$           & 0.0  & 0.0  & \textbf{0.0}    & 0.016             & -0.049            & \textbf{0.0} \\
    $x_{1}\cos(x_{1})$      & 0.0  & 0.0  & \textbf{0.0}    & -0.005            & \textbf{0.0}      & \textbf{0.0} \\
    $x_{1}x_{1}\sin(x_{2})$ & 0.0  & 0.0  & -0.003          & \textbf{0.0}      & \textbf{0.0}      & \textbf{0.0} \\
    $x_{1}x_{2}\sin(x_{1})$ & 0.0  & 0.0  & \textbf{0.0}    & -0.007            & \textbf{0.0}      & \textbf{0.0} \\
    $x_{1}x_{2}\sin(x_{2})$ & 0.0  & 0.0  & 0.003           & \textbf{0.0}      & \textbf{0.0}      & \textbf{0.0} \\
    $x_{1}x_{1}\cos(x_{1})$ & 0.0  & 0.0  & \textbf{0.0}    & -0.009            & \textbf{0.0}      & \textbf{-0.003} \\
    $x_{1}x_{1}\cos(x_{2})$ & 0.0  & 0.0  & -0.001          & \textbf{0.0}      & \textbf{0.0}      & \textbf{0.0} \\
    \bottomrule
\end{tabular} 
\caption{
% \red{what supposed to focus eyes on? }
\small{\textbf{GPSINDy learns better coefficients for the predator-prey model.} In this table we compare the coefficients learned by SINDy and GPSINDy with the ground truth coefficients. The bold values show the best learned coefficients compared to the ground-truth coefficients for both $\dot{x}_1$ and $\dot{x}_2$. }}
\label{tab:gpsindy_coeffs_compare}
% \vspace{-2em}
\end{table}
% 
We demonstrate the effectiveness of GPSINDy on 
% various models, including 
the Lotka-Volterra model, a nonholonomic model with unicycle dynamics, and data from the NVIDIA JetRacer. 
% to underscore 
% This latter test underscores GPSINDy's robustness in handling noisy datasets from real-world hardware. 
% 
We benchmark GPSINDy against the SINDy algorithm \cite{sindy_brunton} and a neural network-based method, NNSINDy. 
% 
NNSINDy uses a neural network for data refinement with 32 hidden neurons, trained using the ADAM optimizer, and LASSO for symbolic regression \cite{Kingma2015AdamAM}.
% 
% The neural network used in NNSINDy has two layers with 32 hidden neurons each and is trained using the ADAM optimizer 
% 
% For all experiments,  
We refer to the ground-truth coefficients as $\boldsymbol{\Xi}_{\text{GT}}$ and the learned coefficients as $\boldsymbol{\Xi}_{\text{Learned}}$ for all experiments.

% 
\paragraph*{Experimental Setup} 
% 
In all experiments unless otherwise specified, 
% 
we simulate the system for $30 \si{\second}$ at  
discrete time steps $ t \in \{ t_1, t_2, \dots, t_\tdim \} $ with a $0.1 \si{\second}$ sampling interval. 
% 
We compute the derivatives $ \dot{\boldsymbol{x}}(t) $ using the true dynamics and add noise 
% 
$\boldsymbol{\epsilon} \sim \mathcal{N}\left(0, \sigma^2 \right)$ 
% 
on top of $\boldsymbol{x}(t)$ and $ \dot{\boldsymbol{x}}(t) $ to simulate measurement noise, thereby obtaining $ \boldsymbol{X} $ and $ \dot{\boldsymbol{X}} $. 
% 
We set aside the last 20\% of the simulated data for validation purposes and use the rest for training. 
% 
We smooth $ \boldsymbol{X} $ and $ \dot{\boldsymbol{X}} $ using Gaussian process regression as described in \eqref{eq:X_GP} and \eqref{eq:Xdot_GP} to obtain $ \boldsymbol{X}_{GP} $ and $ \dot{\boldsymbol{X}}_{GP} $ from the training data. 
% 
We compute $ \boldsymbol{\Theta}( \boldsymbol{X}_{GP} ) $ using \eqref{eq:exp_Thetax} and finally, using $\dot{\boldsymbol{X}}_{GP}$ and $ \boldsymbol{\Theta}( \boldsymbol{X}_{GP} ) $, we solve the $ L_1 $-regularized least-squares problem in \eqref{eq:gpsindy} using $\lambda = 0.1$. 
% 
For the baseline NNSINDy, we train a neural network to predict $\dot{\boldsymbol{X}}$ given the observations of $\boldsymbol{X}$ using the training data and apply LASSO regression to discover the coefficients. 

We choose the candidate function library $\boldsymbol{\Theta}( \boldsymbol{X}, \boldsymbol{U} ) $ (unless otherwise specified) such that it consists of polynomial terms up to $3^{\rm rd}$ order, sinusoidal terms ($\sin$ and $\cos$), and combinations of the 
% polynomial and sinusoidal 
aforementioned 
terms. 
For example, 
\begin{equation}
    % \small
    \begin{small}
    \boldsymbol{\Theta}(\boldsymbol{X}, \boldsymbol{U}) = 
    \begingroup % keep the change local
    \setlength\arraycolsep{4pt}
    \begin{bmatrix}
        \; \; \vertbar \; \; & \vertbar    \; \; & \vertbar         \; \; &        \; \; & \vertbar \; \\
        \; \; 1        \; \; & \boldsymbol{X}  \; \; & \boldsymbol{X}^{P_2} \; \; & \cdots \; \; & \sin(\boldsymbol{U}) & \; \; \cdots \; \;  \\ 
        \; \; \vertbar \; \; & \vertbar    \; \; & \vertbar         \; \; &        \; \; & \vertbar \;
    \end{bmatrix}, 
    \endgroup 
    \label{eq:exp_Thetax}
    \end{small}
\end{equation}
where $\boldsymbol{X}^{P_2}$ 
% denote higher order polynomials. 
% 
denotes the quadratic
nonlinearities in the state variable $\boldsymbol{X} $. 
% 
While we have chosen $\boldsymbol{\Theta}$ for the dynamical systems 
% under consideration 
in our experiments, 
% 
in practice, the function library $\boldsymbol{\Theta}(\boldsymbol{X}, \boldsymbol{U})$ could be expanded to include a wider range of nonlinear basis functions tailored to the system in question. 
% 

% Additionally, we elect to use LASSO as in \eqref{eq:gpsindy} for consistent comparison across all experiments. STLS has been shown to yield better results with noise-free data \cite{cortiella_sindy_l1_regularized}, but in practice this approach failed to yield accurate results in the presence of noise. 
% 
% For the Gaussian process regression used in experiments, we use the squared exponential kernel and optimize the hyperparameters via maximum likelihood to smooth the measurements. 
% 
    
% ========================================== % 

\subsection{Lotka-Volterra Model (Predator/Prey)} 

\begin{figure}[!t]
    \centering
    % \includegraphics[width=0.50\textwidth]{images/predator_prey_error_coeff.png}
    \includegraphics[width=0.50\textwidth]{images/unicycle_error_coeff.png}
    \vspace{-0.5em}
    \caption{
    \small{\textbf{GPSINDy outperforms baselines in learning model coefficients for the unicycle model}. Contrast the dynamics learned by SINDy (blue), GPSINDy (orange), and NNSINDy (green) with trials repeated over 40 seeds for each noise standard deviation $ \sigma $. The horizontal axis represents $\sigma$ varying from $0.050$ to $0.25$ and the vertical axis the mean-squared error between the ground-truth coefficients ($\boldsymbol{\Xi}_{\text{GT}}$) and the learned coefficients ($\boldsymbol{\Xi}_{\text{Learned}}$). The ribbon indicates the standard deviation around the mean line; lower overall error is better.
    }}
\label{fig:predator_prey_unicycle_err_coeff}
\end{figure}
% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=0.50\textwidth]{images/predator_prey_error_coeff.png}
%     \includegraphics[width=0.50\textwidth]{images/unicycle_error_coeff.png}
%     \vspace{-0.5em}
%     \caption{
%     \small{\textbf{GPSINDy outperforms baselines in learning model coefficients for the Predator-Prey (top) and the unicycle model (bottom)}. Contrast the dynamics learned by SINDy (blue), GPSINDy (orange), and NNSINDy (green) with trials repeated over 40 seeds for each noise standard deviation $ \sigma $. The horizontal axis represents $\sigma$ varying from $0.050$ to $0.25$ and the vertical axis the mean-squared error between the ground-truth coefficients ($\boldsymbol{\Xi}_{\text{GT}}$) and the learned coefficients ($\boldsymbol{\Xi}_{\text{Learned}}$). The ribbon indicates the standard deviation around the mean line; lower overall error is better.
%     }}
% \label{fig:predator_prey_unicycle_err_coeff}
% \end{figure}

\begin{figure*}[!t]
    \begin{center}
    \includegraphics[width=1\textwidth]{images/fig2.png}
    \end{center}
    \vspace{-1em}
    \caption{\small{\textbf{GPSINDy outperforms baselines on NVIDIA JetRacer trajectories under noisy measurements.} Each subplot represents the NVIDIA JetRacer dataset at different frequencies (Hz). 
    The horizontal axis represents the noise level standard deviations and the vertical axis the log root mean-squared error (RMSE) between the predicted trajectory  
    (from learned system dynamics) 
    and ground-truth states. 
    Lower overall RMSE is better. 
    % Each baseline is shown in a different color, with GPSINDy in red. 
    This figure shows that over 45 rollouts, although SSR Residual (green) sometimes beats GPSINDy (red), GPSINDy achieves the lowest RMSE for the most frequencies and noise levels. 
    % however, it has significantly higher variance, making it unreliable for real-world settings. 
    }} 
    \label{fig:combined_metrics}
\vspace{-1em}
\end{figure*}
% \begin{figure*}[!t]
%     \begin{center}
%     \includegraphics[width=1\textwidth]{images/combined_metrics.png}
%     \end{center}
%     \vspace{-1em}
%     \caption{\small{\textbf{GPSINDy outperforms baselines on NVIDIA JetRacer trajectories under noisy measurements.} Each column represents the NVIDIA JetRacer dataset at different noise levels. 
%     The horizontal axis represents the data frequency (Hz) and the vertical axis the log root mean-squared error (RMSE) between the predicted trajectory  
%     (from learned system dynamics) 
%     and ground-truth states. 
%     Lower overall RMSE is better. 
%     % Each baseline is shown in a different color, with GPSINDy in red. 
%     This figure shows that over 45 rollouts, GPSINDy (red) achieves the lowest RMSE for most frequencies and noise levels. 
%     SSR Residual (yellow) sometimes beats GPSINDy; however, its significantly higher variance makes it unreliable for real-world settings. 
%     % however, it has significantly higher variance, making it unreliable for real-world settings. 
%     }} 
%     \label{fig:combined_metrics}
% \vspace{-1em}
% \end{figure*}

We first consider the problem of identifying the equations of motion for the Lotka-Volterra model \cite{jorgensen_prey_predator}, which can be used to model the population of predator and prey species over time. 
The dynamics of the system are given by
%  
\begin{align}
    \dot{x}_1 = a x_1 - b x_1 x_2,  \hspace{2em} \dot{x}_2 = -c x_2 + d x_1 x_2,  
    \label{eq:predator-prey}
\end{align}
% 
where $x_1$ represents the size of the prey population and $x_2$ represents the size of the predator population, $a = 1.1$ and $b = 0.4$ describe the prey growth rate and the effect of predation upon the prey population, and $c = 1.0$ and $d = 0.4$ describe the predator's death rate and the growth of predators based on the prey population. 
% 
% We first 
% simulated the system for $30 \si{\second}$ 
% using the deterministic system dynamics in \eqref{eq:predator-prey} at 
% % 
% discrete time steps $ t \in \{ t_1, t_2, \dots, t_\tdim \} $ from an initial condition $x_{0} = [10, 5]^{\top}$ with a sampling interval of $0.1 \si{\second}$. 
% 
% 
% We collected the deterministic states $ \boldsymbol{x}(t) $ and 
For this experiment, we 
standardize the data, i.e. normalize it to have zero mean and unit variance, 
% 
% In Gaussian process regression, standardization is helpful as  
% scaled data is more useful for hyperparameter optimization 
% Standardizing both the output and inputs in Gaussian process regression 
% it aligns with the zero mean assumption, 
to improve parameter estimation of covariance functions and mitigate numerical issues associated with inverting ill-conditioned covariance matrices 
\cite{lingmont_thesis}. 
% 
% Additionally, the kernel matrix needs to be inverted in \eqref{eq:gp_marg_likelihood} and may become ill-conditioned if the data are not properly scaled \cite{lingmont_thesis}. 
% 
% We then computed the derivatives $ \dot{\boldsymbol{x}}(t) $ using the truth dynamics and 
% % 
% added noise 
% % 
% $\boldsymbol{\epsilon} \sim \mathcal{N}\left(0, \sigma^2 \right)$ 
% % 
% on top of the standardized $\boldsymbol{x}(t)$ and $ \dot{\boldsymbol{x}}(t) $ to simulate measurement noise, thereby obtaining $ \boldsymbol{X} $ and $ \dot{\boldsymbol{X}} $. 
% % 
% We set aside the last 20\% of the simulated data for validation purposes and used the rest for training. 
% % 
% We smoothed $ \boldsymbol{X} $ and $ \dot{\boldsymbol{X}} $ using Gaussian process regression as described in \eqref{eq:X_GP} and \eqref{eq:Xdot_GP} to obtain $ \boldsymbol{X}_{GP} $ and $ \dot{\boldsymbol{X}}_{GP} $ from the training data and then computed $ \boldsymbol{\Theta}( \boldsymbol{X}_{GP} ) $ from \eqref{eq:exp_Thetax}. 
% % 
% Finally, using   $\dot{\boldsymbol{X}}_{GP}$ and $ \boldsymbol{\Theta}( \boldsymbol{X}_{GP} ) $, we solved the $ L_1 $-regularized least-squares problem in \eqref{eq:gpsindy} using $\lambda = 0.1$. 
% % 
% For the baseline NNSINDy, we trained a neural network predict $\dot{\boldsymbol{X}}$ given the observations of $\boldsymbol{X}$ using the training data. We performed similar LASSO regression as in GPSINDy to discover the coefficients. 

We first compare the learned coefficients  $\boldsymbol{\Xi}$ between SINDy and our proposed approach in Table \ref{tab:gpsindy_coeffs_compare}. 
% 
We observe that the estimates for the parameters $a,b,c$, and $d$ obtained by GPSINDy are generally a closer approximation of the true underlying dynamics and that the coefficients matrix $ \boldsymbol{\Xi} $ learned by GPSINDy is also more sparse than the one learned by SINDy. 
% 
This is because our approach uses Gaussian processes to estimate $ \dot{\boldsymbol{X}} $, which is a smoother approximation of the true derivatives of $ \boldsymbol{X}$ than the one corrupted by noise. 

% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=0.5\textwidth]{images/pred_prey_combined.png}
%     \caption{\textbf{Trajectories based on GPSINDy-coefficients closely align with ground truth trajectory for the predator-prey model.} We qualitatively compare the trajectories generated using coefficients learned from SINDy (blue), NNSINDy (green) and GPSINDy (orange) against the ground truth (black) trajectory for the predator-prey model. The coefficients were learned using data with added noise of $\boldsymbol{\epsilon} \sim \mathcal{N}\left(0, \sigma^2 = 0.05^2 \right)$. The x-axis shows the time and y-axis shows the corresponding states of the predator-prey model. The top figure depicts the $x_1$ trajectories, while the bottom depicts the $x_2$ trajectories. }
%     \label{fig:pred_prey_x1_single} 
%     \vspace{-1em}
% \end{figure}

We also quantitatively compare the performance of SINDy, NNSINDy, and GPSINDy on data corrupted by different levels of noise as shown in Figure \ref{fig:predator_prey_unicycle_err_coeff}. The results show GPSINDy consistently outperforms the baselines across all noise magnitudes, highlighting its robustness in dealing with noisy data.
NNSINDy, constrained by limited data, fails to effectively learn model coefficients. 
% Furthermore, Figure \ref{fig:predator_prey_unicycle_err_coeff} reveals that 
In Figure \ref{fig:predator_prey_unicycle_err_coeff}, the trajectories derived from GPSINDy's learned coefficients align more closely with the ground truth than those of SINDy and NNSINDy. 
While SINDy is effective at low noise levels, it struggles at higher levels.  
Notably, even though neural networks usually demand vast volumes of data, NNSINDy's trajectory for $\boldsymbol{x}_2(t)$ initially aligns aligns well with the ground truth. 
However, NNSINDy eventually deviates for both $ \boldsymbol{x}_1(t) $ and $ \boldsymbol{x}_2(t) $.

% ========================================== % 

\subsection{Unicycle Dynamics (Simulation)} 

We now consider the nonholonomic unicycle system
% . 
% For this experiment, we produced simulation data based on the dynamics of a unicycle system 
\begin{equation}
\begin{aligned}
    \dot{x}_1 & = x_3 \cos(x_4), &
    \dot{x}_2 & = x_3 \sin(x_4), \\
    \dot{x}_3 & = u_1, &
    \dot{x}_4 & = u_2.
\end{aligned}
\end{equation}

% 
We set the control inputs as $u_1(t) = \sin(t)$ and $u_2(t) = \frac{1}{2}\cos(t)$, 
% to perturb the dynamics 
deterministic functions that perturb the dynamics 
% 
from an initial condition $\boldsymbol{x}_{0} = [0, 0, 0.5, 0.5]^{\top}$. 
In practice, any function can be chosen which perturbs the dynamics. 
Unlike the prior experiment, we opt to not standardize the states $ \boldsymbol{x}(t) $ since the data spread was already apt for Gaussian process regression. 
% 
We note that we use polynomial terms up to $1^{\rm st}$ order in $ \boldsymbol{\Theta} ( \boldsymbol{X}_{GP}, \boldsymbol{U} ) $ as each method failed to identify the true coefficients when $3^{\rm rd}$ order terms were included. 
% 

We compare the performance of SINDy, NNSINDy, and GPSINDy on data with varying noise levels in Figure \ref{fig:predator_prey_unicycle_err_coeff}. 
% 
% GPSINDy consistently outperforms the other methods at higher noise levels. 
% While NNSINDy and GPSINDy perform similarly across predator-prey and unicycle systems, SINDy's performance notably degrades for the unicycle system, especially at higher noise levels. 
% The coefficients learned by all methods have significant errors compared to the true system dynamics, indicating model mismatch. 
% However, GPSINDy demonstrates superior ability to learn accurate coefficients, even with complex dynamics like the nonholonomic unicycle system and noise-corrupted measurements.
% 
GPSINDy consistently outperforms other methods at higher noise levels. 
While NNSINDy and GPSINDy perform similarly for both the predator-prey and unicycle systems, SINDy's performance notably degrades for the unicycle system, particularly with increased noise levels. 
% 
All methods show significant errors in learned coefficients compared to true system dynamics, suggesting model mismatch. 
% 
Nevertheless, our results show that GPSINDy learns more accurate coefficients even with complex dynamics like the nonholonomic unicycle system and noise-corrupted measurements.

Additionally, this experiment demonstrates the impact of selecting terms to include in the function library based on system knowledge. 
% 
% We choose the model that minimizes the mean-squared error of the testing data, but the presence of noise could lead to over-fitting the noise to higher order terms. 
% 
The true system dynamics only contain polynomial terms up to the $1^{\rm st}$ order, but when the function library included terms up to the $ 3^{\rm rd  } $ order, each method overfit the model to the noise by assigning larger weights to the higher order terms. 
% 
We also observed this effect in the predator-prey experiment but with greater impact on the unicycle system,
possibly due to approximating trigonometric functions in the true dynamics with Taylor series terms. 
% 
Reducing the order of the function library to $ 1^{ \rm st } $ order improved model fit for all methods. 

% 


% 
\subsection{JetRacer Hardware Demonstration} 

We also test our method on data collected from a NVIDIA JetRacer, a $1/10 
$ scale high speed car. 
% 
% We actuated the car to drive in a figure-8 made up of two circles, $3 \si{\meter}$
% in diameter. 
We drove the car in a figure-8 made up of two circles, $3 \si{\meter}$ in diameter with nominal lap time of $5.5 \si{\second}$ and nominal velocity of $3.4 \si{\meter\per\second}$. 
% 
VICON sensors captured $22.85 \si{\second}$ of the system's motion at discrete timesteps of $0.02 \si{\second}$ (50 Hz) with the control inputs $ \boldsymbol{U} $ saved at the same sampling rate for 45 total runs. 
% 
We define the state $\boldsymbol{X}_i$ at time $t_i$ to be the measured $x_1$ and $x_2$ position in $\si{\meter}$, forward velocity magnitude $v$ of the car in $\si{\meter\per\second}$, and heading angle $ \phi $ (with respect to a global frame) in $\si{\radian\per\second}$. 
% 
% Each state measurement was then stacked as in
We stack each state measurement 
\eqref{eq:X_data} to gather $ \boldsymbol{X} $, after which we approximate $ \dot{\boldsymbol{X}} $ using central finite differencing. 

% As in previous experiments, we split the data for each run into a training and testing set. 
% 
To evaluate performance for varying frequencies and noise levels, we downsample the 50 Hz state and control time histories to 25, 10, and 5 Hz and add noise $\boldsymbol{\epsilon}_{low} \sim \mathcal{N}\left(0, 0.01^2 \right)$ and $\boldsymbol{\epsilon}_{high} \sim \mathcal{N}\left(0, 0.02^2 \right)$ to the state measurements. 
% 
We generate smoothed points $ \boldsymbol{X}_{GP} $ and $ \dot{\boldsymbol{X}}_{GP} $ at the same 
time points for each frequency and 
as well as twice the input frequency to provide more points for symbolic regression. 
% 
Finally, we compute $ \boldsymbol{\Theta}( \boldsymbol{X}_{GP}, \boldsymbol{U} ) $ using the smoothed points 
% 
% We then solved 
and then solve 
the $L_1$-regularized least squares problem in \eqref{eq:gpsindy} to obtain the GPSINDy dynamics model. 
% 

% 
To achieve the best model fit, we tune $\lambda$ individually for SINDy and GPSINDy via cross-validation, starting at $\lambda = 10^{-6}$ and increment logarithmically until reaching $1$. 
% 
Then, we increase $\lambda$ by 10 until all of the coefficients regress to 0. 
% 
We propagate the dynamics for each $\lambda$ and, at the end, select the $\lambda$ for each $\dot{\mathbf{X}}$ that best fit the data. 
% 
Our baselines include 
% Forward Regression Orthogonal Least Squares (FROLS) \cite{frols_billings2013nonlinear}, and 
Stepwise Sparse Regressor (SSR) Coefficient and Residual \cite{ssr_boninsegna2018sparse}, 
algorithms designed to mitigate measurement noise like GPSINDy and serve as suitable benchmarks. 
% 
SSR Coefficient (Coeff) truncates the smallest coefficient at each iteration while SSR Resiesdual (Res) computes multiple models chopping each coefficient, finally choosing the model with the lowest residual error. 
% 
% We considered another SINDy-based method devised for mitigating noise called Forward Regression Orthogonal Least Squares (FROLS), but 
% \cite{desilva2020}
% 
% Like GPSINDy, these algorithms are designed to handle noisy data and serve as suitable benchmarks.  

% In Figure \ref{fig:single_jetracer}, we qualitatively compare the performance of the GPSINDy and SINDy-learned dynamics models using one of the the testing datasets for the JetRacer. 
% % 
% Both GPSINDy and SINDy learn the car's dynamics from the training dataset and predict the figure-8 trajectory from the testing dataset using fixed control inputs. 
% % 
% However, the figure shows that GPSINDy, having learned more accurate model coefficients, yields a trajectory that aligns more closely with the ground truth. 
% 

\begin{figure}[!t]
    \centering
    \includegraphics[width = 0.5\textwidth,]{images/legend_error.png}
    \includegraphics[width = 0.5\textwidth]{images/unicycle_traj_11.png}
    % \vspace{-1em}
    \caption{
    \small{
    \textbf{GPSINDy Trajectories Align Closely with Ground Truth for the Real JetRacer System.} 
    Contrast the Cartesian trajectories predicted from SINDy (blue) and GPSINDy (orange) with the ground truth (black) based on one rollout out of the total collected JetRacer data. 
    % The axes denote the JetRacer's Cartesian coordinates. 
    For this trajectory, 
    the RMSE error norm between the $x_1$ and $x_2$ coordinates for SINDy on the testing data is $1.4\si{\meter\squared}$, while for GPSINDy it is reduced to $0.23\si{\meter\squared}$}. 
    % This outcome underscores GPSINDy's adeptness at modeling dynamics from noise-afflicted real-world data.
    } 
    \label{fig:single_jetracer}
    \vspace{-1em}
\end{figure}

% 
In Figure \ref{fig:combined_metrics}, we show the results for all 45 rollouts for GPSINDy and the aforementioned baselines. 
% 
For the datasets with added noise  
$\boldsymbol{\epsilon}_{low} $ and $\boldsymbol{\epsilon}_{high} $, 
% 
% FROLS performs best among all baselines, and SINDy and SSR Residual also show comparable performance at frequencies below 50 Hz. 
SSR Res shows the lowest error at the lower frequencies, but GPSINDy gives the lowest error at the higher frequencies and its error bars demonstrate lower variance than SSR Res across all frequencies. 
% 
% For the datasets with high added noise  
% $\boldsymbol{\epsilon}_{high} \sim \mathcal{N}\left(0, 0.02^2 \right)$, 
% 
% FROLS again demonstrates best performance, but SINDy and SSR Residual also show competitive results at frequencies below 50 Hz. 
% 
SSR specializes in identifying stochastic dynamical systems, which could explain its superior performance on the most corrupted data, i.e. data with lowest frequency resolution and artificially added noise.  
% 
However, the poor data quality still frequently leads to model mismatch, resulting in the high variance of the SSR Res error bars. 
% 
GPSINDy beats all baselines for all frequencies with no added noise to the collected data, in particular the \textbf{real-world 50 Hz hardware data}. 
% 
% Table \ref{tab:mean_rmse_baselines} shows that GPSINDy achieves 20.78\% lower RMSE error than SINDy, 83.16\% lower error than SSR Coeff, and 82.23\% lower error than SSR Res. 
% 
% GPSINDy has the lowest aggregate prediction error and variance among the chosen baselines. 
% 
% This could be because SSR prunes candidate nonlinear terms  from the function library at every iteration in a deterministic fashion, which cannot “resuscitate” in the next iterations, possibly funneling the solution into a local minimum. Additionally, SSR 

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \begin{table}[!h] 
% \centering 
% \begin{tabular}{@{}lllll@{}}
% \toprule
% \textbf{}                                            & \textbf{GPSINDy}                                               & \textbf{SINDy}                                                 & \textbf{SSR Coeff}                                             & \textbf{SSR Res}                                               \\ \midrule
% \begin{tabular}[c]{@{}l@{}}Mean RMSE \\ $ \pm $ variance \end{tabular} & \begin{tabular}[c]{@{}l@{}}\textbf{11.002}\\ $ \pm $ \textbf{1.525}\end{tabular} & \begin{tabular}[c]{@{}l@{}}13.888\\ $ \pm $ 1.619\end{tabular} & \begin{tabular}[c]{@{}l@{}}65.349\\ $ \pm $ 3.823\end{tabular} & \begin{tabular}[c]{@{}l@{}}61.917\\ $ \pm $ 40.987\end{tabular} \\ \bottomrule 
% \end{tabular}
%     \caption{\small{\textbf{GPSINDy Achieves Lowest Predicted Error Among Baselines 
%     on 
%     % NVIDIA 
%     JetRacer Trajectories 
%     Under Noisy Measurements.} 
%     This table shows the mean RMSE and variance for all frequencies (5, 10, 25, and 50 Hz) and noise levels (no, low, and high noise). Although SSR Residual sometimes beats GPSINDy on lower frequencies as shown in Figure \ref{fig:combined_metrics}, 
%     GPSINDy achieves the lowest overall mean RMSE and variance. }} 
%     \label{tab:mean_rmse_baselines}
%     \vspace{-1em}
% \end{table} 






==> sections/theorem.tex <==
% \subsection{Improving }

\begin{remark}
Kernel selection is crucial to obtaining improved estimates of the derivatives, which directly influence the accuracy of the identified model coefficients. 
% By selecting an appropriate kernel, 
% Assuming that the chosen GP kernel captures the structure of the true dynamics and that in the absence of noise, the SINDy method correctly identifies the nonzero coefficients, 
% estimating derivatives using GPs 
% with SINDy 
% results in a model 
% that more closely matches true dynamics, in expectation, than using finite difference methods.
\end{remark}

% the dynamics are smooth and differentiable 
% the GP kernel and hyperparameters is chosen/optimized appropriately with structure that matches the dynamics 
% the function library $\Theta$ is well-conditioned and the true dynamics lie within the span of $\Theta$ 
% in absence of noise, the SINDy method correctly identifies the nonzero coefficients 

% \begin{proof}
Consider the unknown dynamical system $\dot{ \boldsymbol{x} }(t) = f( \boldsymbol{x} (t))$.  
Noise-free measurements are collected of the state $\boldsymbol{x}(t)$, but the derivatives $\dot{\boldsymbol{x}}(t)$ must be approximated.   
% $ \boldsymbol{y}_i = \boldsymbol{x}(t_i) + \boldsymbol{\epsilon}_i$, where $\boldsymbol{\epsilon}_i \sim \mathcal{N}(0, \sigma^2)$. 
SINDy identifies $f$ by solving $\dot{\boldsymbol{x}} = \boldsymbol{\Theta}(\boldsymbol{x})\boldsymbol{\xi}$, where $\boldsymbol{\Theta}( \boldsymbol{x} )$ is a library of candidate functions and $\boldsymbol{\xi}$ is a sparse coefficient vector.

% \textbf{Finite Differences (FD):} 
\textbf{Derivative Error:} Estimating $\dot{\boldsymbol{x}}$ via finite differencing introduces high variance in the mean square error (MSE) due to noise amplification 
% 
\begin{equation}
    \text{MSE}_{\text{FD}} = \underbrace{O(\Delta t^2)}_{\text{Bias}^2} + \underbrace{\dfrac{2\sigma^2}{(\Delta t)^2}}_{\text{Variance}},    
\end{equation}
which is minimized at an optimal $\Delta t$ but remains significant because variance increases with $1/(\Delta t)^2$. 
% 
% \textbf{Gaussian Processes (GPs):} 
Estimating $\dot{\boldsymbol{x}}$ using GPs yields lower error bias and variance error 
\begin{equation}
    \text{MSE}_{\text{GP}} = \underbrace{O(l^{2m})}_{\text{Bias}^2} + \underbrace{O\left(\dfrac{\sigma^2}{N l^{2}}\right)}_{\text{Variance}},
\end{equation}
where $l$ is the kernel length-scale, $m$ is the kernel differentiability order, and $N$ is the number of data points. By selecting an appropriate $l$ with sufficient $N$, GPs reduce both bias and variance in estimating derivatives $\dot{\boldsymbol{x}}$ compared to finite differencing, which directly impacts the accuracy of the identified model coefficients $\bxi$. 
% 

% \textbf{Impact on SINDy Model:} 
% The estimation error in $\delta_{\dot{x}} = \hat{\dot{\boldsymbol{x}}} -  \dot{\boldsymbol{x}}$ directly impacts the accuracy of the identified model coefficients $\delta_\xi = \hat{\xi} - \xi$ 
% % 
% \begin{equation}
%     \| \delta_{\xi} \|_2 \leq C  \| \delta_{\dot{x}} \|_2,
% \end{equation}
% % 
% where $C$ is a constant dependent on the restricted isometry property of $ \boldsymbol{\Theta}( \boldsymbol{x} ) $  and $\lambda$ used in LASSO \cite{foucart2023sparsity}. If our problem was least-squares, then C would be the condition number of $\boldsymbol{\Theta}(\boldsymbol{x})$. 
% % where 
% % and  $\kappa_{\boldsymbol{\Theta}}$ is the condition number of $\boldsymbol{\Theta}(\boldsymbol{x})$. 
% % 
% Since $\text{MSE}_{\text{GP}} < \text{MSE}_{\text{FD}}$, 
% it follows that 
% % 
% \begin{equation}
%     \mathbb{E}\left[\|f - \hat{f}_{\text{GP}}\|_2^2\right] < \mathbb{E}\left[\|f - \hat{f}_{\text{FD}}\|_2^2\right].
% \end{equation}

% \textbf{Conclusion:} Using Gaussian processes for derivative estimation yields a model closer to the true dynamics than using finite differencing, due to lower estimation errors in $\dot{\boldsymbol{x}}$.
% \end{proof}

% We have the system 

% $$
% \dot{x} = f(x) = \Theta(x) \xi,
% $$

% but we only have estimates  

% $$
% \hat{\dot{x}} = \hat{f}(x) =  \Theta(x) \hat{\xi}.
% $$

% We want to determine error bounds for the accuracy of the model estimate $\hat{f}$, which is determined by the accuracy of the weight vector $\hat{\xi}$. We can estimate $\hat{\xi}$ using least squares, given derivative estimates $\hat{ \dot{ x } }$

% \begin{align} 
% \hat{\xi} & = \red{\left( \Theta(x)^\top \Theta(x) \right)^{-1} \Theta(x)^\top} \hat{\dot{x}}, \\ 
% \hat{\xi} & = \red{\Theta(x)^{+}}  \hat{\dot{x}},
% \end{align} 

% where $\red{\Theta(x)^{+}} = \red{\left( \Theta(x)^\top \Theta(x) \right)^{-1} \Theta(x)^\top}$ is the pseudoinverse of $\Theta(x)$. The true $\xi$ is given by 

% $$
% \xi = \red{\Theta(x)^{+}}  \dot{x} . 
% $$

% The error in the estimate $\hat{\xi}$ is given by $\delta_{ \xi } = \hat{\xi} - \xi$, and the error in the derivative data $\hat{\dot{x}}$ is given by $\delta_{\dot{x}} = \hat{\dot{x}} - \dot{x}$ . Thus, 

% \begin{align} 
% \hat{\xi} - \xi & = \red{\Theta(x)^{+}} ( \hat{\dot{x}} - \dot{x} ), \\ 
% \delta_{\xi} & = \red{\Theta(x)^{+}} \delta_{\dot{x}}. 
% \end{align} 

% Note that $\delta_{\xi}$ is bounded by $\| \red{\Theta(x)^{+}} \| \|\delta_{\dot{x}} \|$ using the properties of norms 

% \begin{align} 
% \| \delta_{\xi} \| & = \| \red{\Theta(x)^{+}} \delta_{\dot{x}} \| \leq \| \red{\Theta(x)^{+}} \| \| \delta_{\dot{x}} \|,  \\ 
% \| \delta_{\xi} \| & \leq \| \red{\Theta(x)^{+}} \| \| \delta_{\dot{x}} \|. 
% \end{align} 

% The error in the model estimate $\hat{f}$ is given by $\delta_f = \hat{f} - f$, leading to 

% \begin{align} 
% \hat{f} - f & = \Theta(x) ( \hat{\xi} - \xi ), \\ 
% \delta_{f} & = \Theta(x) \delta_{\xi}. 
% \end{align} 

% Note that $\delta_f$ is bounded by $\| \Theta(x) \| \| \delta_\xi \|$ similarly using the properties of norms 

% \begin{align} 
% \| \delta_f \| & = \| \Theta(x)  \delta_\xi \| \leq \| \Theta(x) \| \| \delta_\xi \|, \\ 
% \| \delta_f \| & \leq \| \Theta(x) \| \| \delta_\xi \|. 
% \end{align} 

% We can continue bounding $\| \delta_f \|$ by substituting $\| \delta_{\xi} \|$ with its upper bound  

% \begin{align} 
% \| \delta_{f} \| & \leq \| \Theta(x) \| \| \red{\Theta(x)^{+}} \| \| \delta_{\dot{x}} \| .
% \end{align} 

% Finally, substitute $\kappa_{\Theta} = \| \Theta(x) \| \| \red{\Theta(x)^{+}} \|$, where $\kappa_\Theta$ is the condition number of $\Theta(x)$, to arrive at 

% $$
% \| \delta_{f} \| \leq \kappa_{\Theta} \| \delta_{\dot{x}} \| . 
% $$
